The Effect of Dwarf Galaxies on the Tidal Tails of Globular Clusters

The tidal tails of globular clusters have been shown to be sensitive to the external tidal field. We investigate how Galactic globular clusters with observed tails are affected by satellite dwarf galaxies by simulating tails in galaxy models with and without dwarf galaxies. The simulations indicate that tidal tails can be subdivided into into three categories based on how they are affected by dwarf galaxies: 1) dwarf galaxies perturb the progenitor cluster's orbit (NGC 4590, Pal 1, Pal 5), 2) dwarf galaxies perturb the progenitor cluster's orbit and individual tail stars (NGC 362, NGC 1851, NGC 4147, NGC 5466, NGC 7492, Pal 14, Pal 15), and 3) dwarf galaxies negligibly affect tidal tails (NGC 288, NGC 5139, NGC 5904, Eridanus). Perturbations to a cluster's orbit occur when dwarf galaxies pass within its orbit, altering the size and shape of the orbital and tail path. Direct interactions between one or more dwarf galaxies and tail stars lead to kinks and spurs, however we find that features are more difficult to observe in projection. We further find that the tails of Pal 5 are shorter in the galaxy model with dwarf galaxies as it is closer to apocentre, which results in the tails being compressed. Additional simulations reveal that differences between tidal tails in the two galaxy models are primarily due to the Large Magellanic Cloud. Understanding how dwarf galaxies affect tidal tails allows for tails to be used to map the distribution of matter in dwarf galaxies and the Milky Way.

==> Referee_Response.tex <==
We would like to thank the referee for a helpful and constructive report. We very much apreciate the suggestion to explore which satellite is the primary perturber of each cluster. All suggested references were added, typos were corrected, and figures were edited. Additional referee comments have been copied below and our responses, when necessary, are marked with -->.

Referee Report:

The biggest concern I have is that I think the authors work would be a lot more impactful if they were able to determine which dwarfs create the largest perturbations after the LMC. E.g. at the end of paragraph 1 in Section 3.3, they say “NGC 362… appears to have had a direct encounter with a dwarf galaxy”. For the dwarfs which have such direct/large encounters, it would be very useful if you say which these were in a table or in the text. This would give other researchers a better idea which of the dwarfs to worry about. Previously, only the LMC and Sgr have been found to have an effect so it would be great to hear if there are others. This is partially addressed in Figure 6 which shows that the bulk of the effect is due to the LMC. 

If the authors are worried about how to assess which of the many impacts on the stream produces the largest impact, they could use the results of https://ui.adsabs.harvard.edu/abs/2011ApJ...731...58Y/metrics, https://ui.adsabs.harvard.edu/abs/2015MNRAS.450.1136E/abstract which give expressions for the size of these kicks from point masses or Plummer spheres given the closest approach distance and speed. Having a table with the biggest impactor for each stream would be useful.

--> Thank you very much for this suggestion. As the referee indicates, including such information will increase the impact of our paper. We explored several difference methods to illustrate the importance of each satellite on a given cluster's evolution, and consistently found the LMC or SMC are the biggest impactors for each stream. However, this statement does not do justice to some of the more minor interactions that can still perturb a stream. It would perhaps give the false indication that they are the only satellites that need to be considered. We therefore decided to show the orbital energy evolution of each cluster in the Appendix, along with plots of the distance between each cluster and each satellite. A figure for NGC 4147 is included in the main section of the paper, with additional text added to Section3.2 and 4.2. We now more clearly state how each satellite effects the clusters orbit. To better understand how the tails are effected we would also have to consider the orbital evolution of each tail star, however we now highlight this is something best done once a tail feature is observed for one of these systems.

I also have a number of minor suggestions:

Introduction


8)      Final paragraph. In the second last sentence you say the effect of dwarf galaxy encounters on each globular cluster is quantified but you also do it for the tidal streams of these GCs so that would be good to point out.
--> text added

Section 2

3)      Second paragraph, when introducing the hernquist potential for each dwarf, it would be useful to give the mass and scale radius that you use for completeness. If the scale radius is selected in some informative way, i.e. to match the observed velocity dispersion at some distance, that would also be good to point out.
--> We now list the masses and scale radii used for our models
4)      Second paragraph, it would be useful for completeness to state here whether you allow the Milky Way to move in response to these dwarfs (especially the LMC) --> made clarification and was previously mentioned in conclusion 
--> We state specifically now that the Milky Way remains fixed. As we note in the conclusion, accounting for the Milky Way's response to its satellites is a necessary next step
5)        Last paragraph, when mentioning the rewinding, this is presumably done in the presence of each dwarf so that the GC ends up in the right place when integrated forwards. It would be useful to point that out.
--> We now state more clearly that the dwarf galaxies are moving in the DG galaxy model and that the cluster's end up in the correct final position.
6)      In this section it would be good to know if you did any Monte Carlo for the orbital uncertainties of each dwarf and GC or if you selected the median values from the observed pms, distances, rvs and used these.
--> We now state explicitly that we use the mean values quoted by the Gaia Collaboration

Section 3

1)      Section 3.2, second paragraph, last sentence. It would be good to know how close this encounter was and, if possible, the relative velocity at that point.
--> Text added
2)      Section 3.2, third paragraph. In this paragraph, you discuss a lot of interesting encounters. As I mentioned above, it would be great if there was a table here with which dwarf produced the largest perturbation for each stream. That could be estimated with the references given in the main suggestion given above.
--> Some additional text in Section 3.2 and a new figure have been added to address this comment
3)      Section 3.3, first paragraph, last sentence. Which dwarf was this? That would be good to know.
--> We point out that it can't be known for certain which dwarf is responsible for the feature, but we do list candidates
4)      Section 3.3, second paragraph. When discussing the spurs of Pal 14, it would again be good to know which dwarf did this.
--> We point out that it can't be known for certain which dwarf is responsible for the feature, but we do list candidates

5)      Section 3.4, first paragraph. Here you say that the perturbation must be visible on the plane of the sky and you show plots of the positions of the stream. It may be good to point out that perturbations in streams can be identified in velocity space (i.e. with stream velocities that aren’t aligned with the stream https://ui.adsabs.harvard.edu/abs/2019MNRAS.487.2685E/abstract). 
--> Text added to Section 3.4


Section 4

1)      Section 4.2, second paragraph. Here it would be good to state whether you allow the Milky Way to move in response to the LMC (e.g. https://ui.adsabs.harvard.edu/abs/2015ApJ...802..128G/abstract, https://ui.adsabs.harvard.edu/abs/2019MNRAS.487.2685E/abstract) 
--> mentioned in conclusion, with additiona text added to Section 2.

==> notes.tex <==
%% Define notes using todonotes package

\usepackage{xparse}
\usepackage{ifthen}

\makeatletter
% Increase margins for margin comments
\ifthenelse{\@todonotes@enable=1 \AND \@todonotes@inline=0}{
\paperwidth=\dimexpr\paperwidth + 6cm\relax
%\textwidth=\dimexpr \textwidth - 6cm\relax
\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
\marginparwidth=\dimexpr \marginparwidth + 2.5cm\relax}{}

\ifthenelse{\@todonotes@enable=1}
  {\usepackage[textwidth=\dimexpr\evensidemargin + 2.25cm]{todonotes}}
  {\usepackage[disable]{todonotes}}

% Colors for comment boxes
\definecolor{gold}{RGB}{255,215,0}
\definecolor{salmon}{rgb}{0.95,0.5,0.25}
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{darkblue}{rgb}{0.0, 0., 0.7}
\definecolor{vlightblue}{rgb}{0.68,0.84,0.9}
\definecolor{purple}{rgb}{0.7, 0., 0.7}
\definecolor{lavender}{rgb}{0.9, 0.9, 0.98}

\newcommand{\@todonotes@loaded}{0}
\@ifpackageloaded{todonotes}
  {\renewcommand{\@todonotes@loaded}{1}}
  {\renewcommand{\@todonotes@loaded}{0}}
% Deal with inline: hack
\ifthenelse{\@todonotes@inline=0}
  {\renewcommand{\@todonotes@loaded}{1}}
  {\renewcommand{\@todonotes@loaded}{0}}
\@ifpackagewith{todonotes}{disable}
  {\renewcommand{\@todonotes@loaded}{0}}
  {}

% Increase margins for margin comments
%\ifthenelse{\@todonotes@loaded=1}{
%\textwidth=\dimexpr \textwidth - 6cm\relax
%\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
%\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
%\marginparwidth=\dimexpr \marginparwidth + 2.5cm\relax}{}

\ifthenelse{\@todonotes@inline=1}{
\NewDocumentCommand{\note}{O{black} O{gold} m}{\todo[inline,backgroundcolor={#2},linecolor={#2},bordercolor={#1}]{{\protect\footnotesize #3}}}}
{\NewDocumentCommand{\note}{O{black} O{gold} m}{\todo[backgroundcolor={#2},linecolor={#2},bordercolor={#1}]{{\protect\footnotesize #3}}}}
\makeatother
